Termination Criteria for Solving Concurrent Safety and Reachability Games

We consider concurrent games played on graphs. At every round of a game, each player simultaneously and independently selects a move; the moves jointly determine the transition to a successor state. Two basic objectives are the safety objective to stay forever in a given set of states, and its dual, the reachability objective to reach a given set of states. We present in this paper a strategy improvement algorithm for computing the value of a concurrent safety game, that is, the maximal probability with which player~1 can enforce the safety objective. The algorithm yields a sequence of player-1 strategies which ensure probabilities of winning that converge monotonically to the value of the safety game. Our result is significant because the strategy improvement algorithm provides, for the first time, a way to approximate the value of a concurrent safety game from below. Since a value iteration algorithm, or a strategy improvement algorithm for reachability games, can be used to approximate the same value from above, the combination of both algorithms yields a method for computing a converging sequence of upper and lower bounds for the values of concurrent reachability and safety games. Previous methods could approximate the values of these games only from one direction, and as no rates of convergence are known, they did not provide a practical way to solve these games.

==> strategy-improve.tex <==
\section{Strategy Improvement Algorithm}
In this section we present a strategy improvement (aka policy iteration) 
algorithm~\cite{HofKar66} for concurrent games with reachability 
objectives. 
Let $W_1=\set{s \in S \mid \va(s)=1}$ be the set of states with value~1 for 
player~1.
Recall $W_2=\set{s\in S \mid \va(s)=0}$.
The sets $W_1$ and $W_2$ can be computed in time quadratic in the size of 
the game graph by symbolic algorithms~\cite{luca-focs98}.
Also it easily follows that for all states $s \in S$ we have 
$\va(s)=\vaw(s)$.
Hence we assume that all states in $W_1 \cup W_2$ are converted to 
absorbing states and compute $\vaw(s)$ to compute $\va(s)$.
We present some preliminary notations before we present the algorithm.

\begin{definition}[Proper strategies]
A memoryless strategy $\stra_1$ is a \emph{proper strategy} for 
player~1 if for every pure memoryless strategy $\stra_2$ for player~2 and
for all states $s \in S \setminus \wab$ we have 
$\Prb_s^{\stra_1,\stra_2}(\Reach(\wab))=1$.
\end{definition} 


\begin{lemma}\label{lemm:proper1}
Let $\stra_1$ be a proper strategy.
Then for all strategies $\stra_2$ for player~2 and for all states 
$s \in S \setminus \wab$ we have $\Prb_s^{\stra_1,\stra_2}(\Reach(\wab))=1$.
\end{lemma}
\begin{proof}
Given the memoryless strategy $\stra_1$ consider the player 2-MDP $G_{\stra_1}$
with the safety objective $\Safe(S \setminus \wab)$.
If there is a strategy $\stra_2$ and a state $s \in S \setminus \wab$ such
that $\Prb_s^{\stra_1,\stra_2}(\Safe(S \setminus \wab))>0$,
then there is a pure memoryless strategy $\stra_2^*$ such that 
$\Prb_s^{\stra_1,\stra_2^*}(\Safe(S \setminus \wab))>0$, since 
pure memoryless optimal strategies exist in MDPs with 
safety objectives~\cite{FilarVrieze97}.
This contradicts that $\stra_1$ is proper.
\qed
\end{proof}

\begin{lemma}\label{lemm:proper2}
Let $\stra_1^*$ be the memoryless strategy such that for all $s \in S \setminus 
\wab$ the strategy $\stra_1^*$ plays all moves in $\mov_1(s)$ 
uniformly at random.
Then $\stra_1^*$ is a proper strategy.
\end{lemma}
\begin{proof}
Assume towards contradiction that $\stra_1^*$ is not proper.
Then there is a state $s \in S \setminus \wab$ and a pure memoryless 
strategy $\stra_2^*$ such that 
$\Prb_s^{\stra_1^*,\stra_2^*}(\Safe(S \setminus \wab))>0$.
Then there must exist a closed recurrent set $C \subseteq S \setminus \wab$ 
in the Markov chain $G_{\stra_1^*,\stra_2^*}$.
Given $\stra_2^*$ consider the player 1-MDP $G_{\stra_2^*}$.
For every  memoryless strategy $\stra_1$ for player~1 and for all 
states $s \in C$ we have 
$\Prb_s^{\stra_1,\stra_2^*}(\Safe(C))
\geq \Prb_s^{\stra_1,\stra_2^*}(\Safe(S \setminus W_1))=1$.
This follows since $\supp(\stra_1(s)) \subs \supp(\stra_1^*(s))$ for all 
$s \in C$.
Since pure memoryless optimal strategies exists in MDPs with reachability
objectives~\cite{FilarVrieze97}, it follows that $\stra_2^*$ is a 
witness optimal strategy for all states $s \in C$ to show that $\va(s)=0$.
This is a contradiction as this would mean $C \subseteq W_2$ and we 
started with the assumption that $C \subseteq S \setminus \wab$.
\qed
\end{proof}


\paragraph{Ordering of strategies.}
We define a pre-order $\prec$ on the strategies as follows:
given two strategies $\stra_1$ and $\stra_1'$ we have 
$\stra_1 \prec \stra_1'$ iff the following conditions hold:
(a)~$\vas{\stra_1} \leq \vas{\stra_1'}$ and 
(b)~$\vas{\stra_1}(s) < \vas{\stra_1'}(s)$ for some state $s$.
Given two strategies $\stra_1$ and $\stra_1'$ we denote by 
$\stra_1 \preceq \stra_1'$ that either $\stra_1 \prec \stra_1'$ or 
$\stra_1 = \stra_1'$.


\paragraph{Informal description of Algorithm~\ref{algorithm:strategy-improve}.}
We now present the strategy improvement algorithm 
(Algorithm~\ref{algorithm:strategy-improve}) for computing the values for 
states in $S \setminus \wab$.
The algorithm iteratively improves strategies according to the pre-order 
$\prec$. 
An informal description of the algorithm is as follows:
the algorithm starts with the initial strategy $\stra_1^0=\stra_1^*$ as 
described in Lemma~\ref{lemm:proper1}.
At iteration $i+1$ it considers the memoryless strategy $\stra_1^i$ and 
the computes the values $\vas{\stra_1^i}$.
Observe that since $\stra_1^i$ is a memoryless strategy the computation of 
$\vas{\stra_1^i}$ involves solving the player $2$-MDP $G_{\stra_1^i}$.
The value $\vas{\stra_1^i}$ is denoted as the valuation $v_i$.
For all states $s$ such that $\Pre_1(v_i)(s) > v_i(s)$, 
the memoryless strategy at $s$ is modified to a selector $\zeta_{i+1}$ 
obtained as the optimal selector for $\Pre_1(v_i)(s)$, i.e.,
$\Pre_{1: \zeta_{i+1}}(v_i)(s) = \Pre_1(v_i)(s)$.
The algorithm then proceeds to the next iteration.
If for all states $s$ we have $\Pre_1(v_i)(s)=v_i(s)$, then the algorithm 
stops and returns the strategy $\stra_1^i$.


\begin{algorithm*}[t]
\caption{Strategy Improvement Algorithm}
\label{algorithm:strategy-improve}
{
\begin{tabbing}
aa \= aa \= aaa \= aaa \= aaa \= aaa \= aaa \= aaa \kill
\\
\> {\bf Input :} A concurrent game $G$ with sets $W_1$ and $W_2$. \\
\>   {\bf Output:} A strategy $\stra_1$ for player~1. \\ 

\> 1. Consider $\stra_1^0=\stra_1^*$ such that for all 
	$s \in S \setminus \wab$ \\
\>\>  the strategy $\stra_1^0$ plays all moves in $\mov_1(s)$ uniformly at 
	random. \\
\> 2. $i=0$, and compute $v_0 = \vas{\stra_1^0}$. \\

\> 3. {\bf do \{ } \\ 
\>\> 3.1. let $I= \set{s \in S \setminus \wab \mid \Pre_1(v_i)(s) > v_i(s)}$. \\
\>\> 3.2. Let $\zeta_{i+1}$ be a selector such that for all states $s \in I$ 
	we have $\Pre_{1:\zeta_{i+1}}(v_i)(s) =\Pre_1(v_i)(s) > v_i(s)$.\\
\>\> 3.3. The memoryless strategy $\stra_1^{i+1}$ is defined as follows: for a 
	state $t$ we have\\
\>\>\> $	\displaystyle 
	\stra_1^{i+1}(t)=
	\begin{cases}
	\stra_1^i(t) & s\not\in I;\\
	\zeta_{i+1}(s) & s\in I.
	\end{cases}$
	\\ \\ 
\>\> 3.4. $v_{i+1} =\vas{\stra_1^{i+1}}$; \\
\>\> 3.5. $i=i+1$. \\
\>\> {\bf \} while } ($I\neq \emptyset$)  ({\bf end do})\\ \\

\> 4. {\bf return} $\stra_1^{i}$.

\end{tabbing}
}
\end{algorithm*}




\begin{lemma}\label{lemm:proper3}
Let $\stra_1^i$ and $\stra_i^{i+1}$ be strategies obtained at iteration 
$i$ and iteration $i+1$ of Algorithm~\ref{algorithm:strategy-improve}.
If $\stra_1^i$ is a proper strategy, then $\stra_1^{i+1}$ is also a
proper strategy. 
\end{lemma}
\begin{proof}
Assume towards contradiction that $\stra_1^i$ is a proper strategy and 
$\stra_1^{i+1}$ is not a proper strategy.
Let $\stra_2^*$ be a pure memoryless strategy for player~2 
to witness that $\stra_i^{i+1}$ is not a proper strategy.
Then there exist $C \subseteq S \setminus \wab$ such that $C$ is closed 
recurrent set of states in the Markov chain $G_{\stra_1^{i+1},\stra_2^*}$.
Let $I$ be the non-empty set of states where the selector is modified to 
obtain $\stra_1^{i+1}$ from $\stra_1^i$, and at all other states the strategies 
$\stra_1^i$ and $\stra_1^{i+1}$ agree.
We denote by $\zeta_i,\zeta_{i+1}$ and $\zeta_*$ the selectors corresponding 
to the strategies $\stra_1^i,\stra_1^{i+1}$ and $\stra_2^*$, respectively.

 Since $\stra_1^i$ and $\stra_1^{i+1}$ agree at all states other than the
states in $I$
and $\stra_1^i$ is a proper strategy it follows that we must have $C \cap I 
\neq \emptyset$.
Let $U_r^i =\set{s \in S \setminus \wab \mid \vas{\stra_1^i}(s)=v_i(s)=r}$
be the value class with value $r$ at iteration $i$.
For a state $s \in U_r^i$ the following assertion hold: 
if $\dest(s,\zeta_i,\zeta_*) \subsetneq U_r^i$, then 
$\dest(s,\zeta_i,\zeta_*) \cap U_{>r}^i \neq \emptyset$.
Let $z =\max\set{r \mid U_r^i \cap C \neq \emptyset}$, i.e.,
$U_z^i$ is the greatest value class of iteration $i$ with non-empty 
intersection with the closed recurrent set $C$.
It easily follows that $0 < z <1$. 
Consider $s^* \in I$ and let $s^* \in U_q^i$. 
Since $\Pre_1(v_i)(s^*) > v_i(s^*)$, it follows that 
$\dest(s^*,\zeta_{i+1},\zeta_*) \cap U_{>q}^i \neq \emptyset$.
Hence we must have $z >q$ and hence we have 
$I \ \cap \ C \ \cap U_z^i =\emptyset$.
Thus for all states 
$s \in U_z^i \cap C$ we have $\stra_1^i(s)=\stra_1^{i+1}(s)$.
Recall $z$ is the greatest value class of iteration $i$ with non-empty 
intersection with $C$; hence $U_{>z}^i \cap C=\emptyset$.
Thus for all states $s \in C \cap U_z^i$ we have 
$\dest(s,\zeta_i,\zeta_*) \subseteq U_i^z \cap C$.
It follows that $C \subseteq U_z^i$.
However, this gives us a contradiction that $C \cap I \neq \emptyset$, 
$I \cap C \cap U_z^i =\emptyset$ and $C \subseteq U_z^i$.
\qed
\end{proof}


\begin{lemma}\label{lemm:proper4}
For all $i\geq 0$, a strategy $\stra_1^i$ obtained at iteration $i$ of 
Algorithm~\ref{algorithm:strategy-improve} is a proper strategy.
\end{lemma}
\begin{proof}
By Lemma~\ref{lemm:proper2} we have $\stra_1^0$ is a proper strategy.
The rest follows from Lemma~\ref{lemm:proper3} and induction.
\qed
\end{proof}

\begin{lemma}\label{lemm:stra-improve}
Let $\stra_1^i$ and $\stra_1^{i+1}$ be strategies obtained at 
iteration $i$ and iteration $i+1$ of Algorithm~\ref{algorithm:strategy-improve}
for $i \geq 0$.
Let $I=\set{s \in S \mid \Pre_1(v_i)(s) > v_i(s)}$.
Let $v_i=\vas{\stra_1^i}$ and $v_{i+1}=\vas{\stra_1^{i+1}}$.
Then the following assertion hold:
\[
v_{i+1}(s)  \geq  \Pre_1(v_i)(s); \qquad \forall s \in S;
\]
and hence
\[
\begin{array}{rcll}
v_{i+1}(s) & \geq & v_i(s);  & \forall s \in S; \\
v_{i+1}(s) & > & v_i(s);  & \forall s \in I.
\end{array}
\]
\end{lemma}
\begin{proof}
Consider the valuation $v_i$ and $v_{i+1}$ obtained at iteration $i$ and 
$i+1$, respectively.
Let $w_i=1-v_i$ be the valuation obtained by subtracting the valuation $v_i$
from~1.
Since $\stra_1^{i+1}$ is a proper strategy (by Lemma~\ref{lemm:proper4}),
it follows that the counter-optimal strategy for player~2 to minimize
$v_{i+1}$ is obtained by maximizing the probability to reach $W_2$.
Hence we consider the player 2-MDP $G_{\stra_1^{i+1}}$ with the 
reachability objective $\Reach(W_2)$ for player~2.
Let $\zeta_i$ and $\zeta_{i+1}$ be the selectors corresponding the memoryless
strategies $\stra_1^i$ and $\stra_1^{i+1}$, respectively.
Let $w_{i+1}(s)=w_i(s)$ for all $s \in S \setminus I$ and 
$w_{i+1}(s^*)=1-\Pre_1(v_i)(s^*) < w_i(s^*)$ for all states $s^* \in I$.
In other words, $w_{i+1} = 1 -\Pre_1(v_i)$ and we also have $w_{i+1} \leq w_i$.
We now show that $w_{i+1}$ is a feasible solution to the 
linear-program for MDPs with reachability objectives as described in 
subsection~\ref{subsec:mdpreach}.
Since $v_i =\vas{\stra_1^i}$ it follows that
\[
w_i(s) \geq \sum_{t \in S} w_i(t) \cdot \trans_{\zeta_i}(s,b); 
\qquad \forall b \in \mov_2(s); \forall s\in S.
\]
For all states $s \in S \setminus I$ we have $\zeta_i(s)=\zeta_{i+1}(s)$ and
$w_{i+1}(s)=w_i(s)$,
and since $w_{i+1} \leq w_i$ it follows that for all $s \in S \setminus I$ 
we have
\[
w_{i+1}(s) \geq \sum_{t \in S} w_{i+1}(t) \cdot \trans_{\zeta_{i+1}}(s,b); 
\qquad \forall b \in \mov_2(s).
\]
Since the selector $\zeta_{i+1}(s^*)$ is obtained as an optimal
selector for $\Pre_1(v_i)(s^*)$ for all states $s^* \in I$,
the following assertion hold:
\[
w_{i+1}(s^*) \geq \sum_{t \in S} w_{i}(t) \cdot \trans_{\zeta_{i+1}}(s^*,b); 
\qquad \forall b \in \mov_2(s^*); \forall s^* \in I.
\] 
Since $w_{i+1} \leq w_i$, the following inequalities are immediate
\[
w_{i+1}(s^*) \geq \sum_{t \in S} w_{i+1}(t) \cdot \trans_{\zeta_{i+1}}(s,b); 
\qquad \forall b \in \mov_2(s^*); \forall s^* \in I.
\] 
Hence it follows that $w_{i+1}$ is a feasible solution to the 
linear-program for MDPs with reachability objectives as described in 
subsection~\ref{subsec:mdpreach}.
Since the reachability valuation for player~2 for $\Reach(W_2)$ is the least
solution (observe the objective function of the linear-program is a 
minimizing function), it follows that 
$v_{i+1} \geq 1-w_{i+1} = \Pre_1(v_i)$; and thus we obtain
$v_{i+1}(s) \geq v_i(s)$ for all $s \in S$ and 
$v_{i+1}(s^*) > v_i(s^*)$ for all $s^* \in I$.
\qed
\end{proof}


\begin{theorem}[Strategy improvement]\label{thrm:stra-improve}
The following assertions hold.
\begin{enumerate}
\item 
For all $i \geq 0$ we have $\stra_1^i \preceq \stra_1^{i+1}$ and 
if $\stra_1^i = \stra_1^{i+1}$ is an optimal strategy.


\item $\lim_{i \to \infty} v_i =
\lim_{i \to \infty} \vas{\stra_1^i} = \va$.

\end{enumerate}
\end{theorem}
\begin{proof}
We prove the results as follows.
\begin{enumerate}
\item The result that $\stra_1^i \preceq \stra_1^{i+1}$ follows from 
Lemma~\ref{lemm:stra-improve}.
If $\stra_1^i =\stra_1^{i+1}$, then we have 
$\Pre_1(v_i)=v_i$.
Consider a selector $\zeta_2$ for player~2 such that 
$\Pre_1(v_i)=\sup_{\zeta_1 \in \Sel_1} \Pre_{\zeta_1,\zeta_2}(v_i)$.
The memoryless strategy $\stra_2^*$ that plays the selector $\zeta_2$ 
is an optimal strategy for player~2 and ensures that 
$\vaw \leq \vas{\stra_1^i}$.
Since $\vas{\stra_1^i} \geq \vaw$ it follows that $\stra_1^i$ is an 
optimal strategy for player~1.

\item  Let $v_0= [W_1]$ and $u_0=[T]$.
We have $u_0 \leq v_0$.
For all $k\geq 0$, by Lemma~\ref{lemm:stra-improve} we have 
$v_{k+1} \geq [W_1] \lor \Pre_1(v_k)$.
For all $k \geq 0$, let $u_{k+1}=[T] \lor \Pre_1(u_k)$.
Thus by induction we conclude for all $k \geq 0$ we have $u_k \leq v_k$.
Moreover, $v_k \leq \vaw$, 
i.e., for all $k\geq 0$, we have $$u_k \leq v_k \leq \vaw =\va.$$
Since $\lim_{k \to \infty} u_k = \va$ it follows that
\[
\lim_{k \to \infty} \vas{\stra_1^k}= \lim_{k \to \infty} v_k= \va.
\] 
\end{enumerate}
The desired result follows.
\qed
\end{proof}


\paragraph{Termination for $\vare$-approximation.}
We now present two conditions for the termination of the strategy improvement 
algorithm for $\vare$-approximations. 
We presented Algorithm~\ref{algorithm:strategy-improve} to obtain 
under approximations $\vas{\stra_1^i}$ for values $\va$ for player~1.
Symmetrically we can obtain a strategy improvement 
algorithm (say Algorithm~2) to obtain under approximations 
$\vbs{\stra_2^i}$ for values $\vb$ for player~2.
Then Algorithm~\ref{algorithm:strategy-improve} and Algorithm~2 can 
be dove-tailed and the following result presents a criteria to terminate 
for $\vare$-approximation.

\begin{theorem}
Let $\vas{\stra_1^i}$ and $\vbs{\stra_2^i}$ be the values for player~1 
and player~2 obtained at iteration $i$ 
of Algorithm~\ref{algorithm:strategy-improve} and Algorithm~2, respectively.
For $\vare>0$, if 
\[
\bigg(1 -\vbs{\stra_2^i}(s)\bigg) - \vas{\stra_1^i}(s) \leq \vare,
\] 
then $\vas{\stra_1^i}(s)\geq \va(s) - \vare$, and 
$\stra_1^i$ is an $\vare$-optimal strategy for state $s$. 
\end{theorem}


\paragraph{Approximation by $k$-uniform strategies.}
A memoryless strategy $\stra_1$ is a $k$-uniform memoryless strategy if for 
all $s \in S \setminus \wab$, for all $a \in \supp(\stra_1(s))$, 
there exists $i,j \in \Nats$ such that $0 \leq i \leq j \leq k$ and
$\stra_1(s)(a)=\frac{i}{j}$, i.e., the moves in the support are  played 
with probability that are multiples of $\frac{1}{\ell}$ with $\ell \leq k$.
The results of~\cite{CMJ04} establishes that for all $\vare>0$, there 
exists $k$-uniform memoryless $\vare$-optimal strategy for 
$k=\frac{\big(192\cdot |S|^4\cdot \ln (4|\trans|)\big)}{\vare^2}$.
The number of $k$-uniform memoryless strategies are bounded by 
$k^{(2\cdot |\trans|)}$.
The strategy improvement of Algorithm~\ref{algorithm:strategy-improve} can
be restricted to $k$-uniform memoryless strategies and an $\vare$-optimal
strategy can be obtained in $k^{(2\cdot |\trans|)}$ iterations, where 
$k=\frac{\big(192\cdot |S|^4\cdot \ln (4|\trans|)\big)}{\vare^2}$.
The following bound on Algorithm~\ref{algorithm:strategy-improve} (without 
the restriction of strategy improvement with $k$-uniform memoryless strategies)
is an immediate consequence.


\begin{theorem}
For $\vare>0$, 
let $k=\frac{\big(192\cdot |S|^4\cdot \ln (4|\trans|)\big)}{\vare^2}$ and 
$i= k^{(2 \cdot |\trans|)}$.
Let $\stra_1^i$ be the strategy obtained at iteration $i$ of 
Algorithm~\ref{algorithm:strategy-improve},
then $\stra_1^i$ is an $\vare$-optimal strategy for all states in 
$S \setminus \wab$ for the objective 
$\Reach(W_1)$. 
\end{theorem} 

